Physics-Guided Deep Neural Networks for Power Flow Analysis

Solving power flow (PF) equations is the basis of power flow analysis, which is important in determining the best operation of existing systems, performing security analysis, etc. However, PF equations can be out-of-date or even unavailable due to system dynamics and uncertainties, making traditional numerical approaches infeasible. To address these concerns, researchers have proposed data-driven approaches to solve the PF problem by learning the mapping rules from historical system operation data. Nevertheless, prior data-driven approaches suffer from poor performance and generalizability, due to overly simplified assumptions of the PF problem or ignorance of physical laws governing power systems. In this paper, we propose a physics-guided neural network to solve the PF problem, with an auxiliary task to rebuild the PF model. By encoding different granularity of Kirchhoff's laws and system topology into the rebuilt PF model, our neural-network based PF solver is regularized by the auxiliary task and constrained by the physical laws. The simulation results show that our physics-guided neural network methods achieve better performance and generalizability compared to existing unconstrained data-driven approaches. Furthermore, we demonstrate that the weight matrices of our physics-guided neural networks embody power system physics by showing their similarities with the bus admittance matrices.

==> ack.tex <==
\section*{Acknowledgment}
\iffalse
The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.
\fi

==> code/fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> datadriven-vs-numeric.tex <==
\subsection{Data-driven Solver versus Numerical Solver}


==> new-storyline.tex <==
\section{Introduction}
\begin{enumerate}
   % 1st paragraph
   \item Power Flow Analysis Introduction \& Conventional Methods:
   \begin{itemize}
     \item The definition of power flow analysis.\\
     Power-Flow (PF) analysis is to determine the power system's steady state operating condition in terms of the voltage magnitude and phase angles at each bus for specified load, generator real power and voltage conditions~\cite{saadat1999power}. 
     \item The importance of power flow analysis.
     \item Conventional methods to solve power flow problem: state-space method (DAE models described in mathematical equations) + numerical method to solve the equations.
   \end{itemize}
    % 2nd paragraph
   \item Problems of Conventional Methods: no accurate DAE model, thus power flow solutions are inaccurate (Goal: Introducing why need data-driven/machine-learning methods):
   \begin{itemize}
       \item \textbf{Dynamics, uncertainties, limited knowledge} of modern power systems make it \textbf{difficult} to obtain \textbf{ accurate mathematical equations}. 
       \begin{itemize}
           \item Distributed Energy Resources are too volatile and uncertain (not-well-understood) to be precisely expressed by equations.
           \item The system parameters are inaccurate(by aging, weathering), unknown line profiles in secondary distributed systems. \\
           NOTE: DON'T say `system evolving', `equation/model updating', otherwise, reviewer will assume/expect our methods is adaptive to changes, instead talk `adaptive' in discussion and future work.
       \end{itemize}
       \item The consequences of inaccurate DAE model?
       \begin{itemize}
           \item blackout~\cite{liscouski2004final,ferc2012arizona}.
           \item Difficult to integrate DERs, and thus affect stability, sustainability~\cite{yu2017patopa, yu2017data}.
       \end{itemize}
   \end{itemize}
   % 3rd and 4th paragraph
   \item Data-driven methods to do power flow analysis. 
   \begin{itemize}
       \item \textbf{learn parameters to calibrate DAE models + numerical solutions}.
       \begin{itemize}
           \item Related work: learn line parameters~\cite{yu2017data};learn Power Flow Jacobian Matrix
           \item \textbf{Disadvantages}:\\
           a) numerical method is computational expensive (need citation), and not stable depending on initialization;\\
           b) Error Accumulation: Estimation errors from learning + Approximation errors from numerical solution.Experiments results show MAPE $>$=3\% parameter estimation error cause huge numerical errors.\\
           NOTE: may need to compare the computation time and accuracy with our methods.
       \end{itemize}
       \item \textbf{ use machine learning to solve power flow model/DAEs by inferring the mapping rules between the observed inputs-outputs of systems}.
       \begin{itemize}
           \item Related work: LR to build the power flow model and solve it; SVR to build the power flow model and solve voltage magnitude.
           \item \textbf{Disadvantages/Challenges}:\\
           a) non-linearity;\\
           b) noise and outliers in measurement data;\\
           c) algorithm's scalability;\\
           d) \textbf{respect the physical laws}. \\
       \end{itemize}
   \end{itemize}
   % 5th paragraph
   \item Introduce our methods:
   \begin{itemize}
       \item Methods design insights and principles:\\
       a) Power flow solutions are no guaranteed to be unique. The inverse function of quadratic/trigonometric equations does not exist, no-closed form of power flow solutions\\
       b) Neural networks are universal `function' approximator. Related work: Neural networks are used to solve differential equations, to find roots of polynomial and linear equations~\cite{huang2004constructive}.\\
       TODO: read ~\cite{huang2004constructive} more thoroughly.\\
       c) Add physical laws to constrain neural networks, since there are no specific/accurate power flow equations for NN to solve.\\
       d) Stop criteria of Newton's method(iterative numerical methods) is similar to Auto-Encoder's reducing reconstruction error.
       \item At high-level, how our methods leverage the insights and principles to solve the problems:\\
       Inspired by the Auto-Encoder,\\
       a) we utilize a MLPNN as `encoder' to solve power flow problem by inferring the mapping rules from the known variables of power flow model to the bus voltages.\\
       b) Impose physical laws on the MLPNN `encoder':\\
       \begin{itemize}
           \item \textbf{Implicit physical laws learned from data}: utilize another MLPNN as `decoder' to learn the power flow model from data by inferring the mapping rules from the bus voltages to power injections. 
           \item \textbf{Kirchhoff's laws:} design a BNN as `decoder' to learn the quadratic power flow model from data.
       \end{itemize}
       c) Multiple objectives in training:\\
       i) minimize differences between the voltage solutions obtained by MLPNN `encoder' and the voltage measurements in training data;\\
       ii) minimize differences between the power injections reconstructed by the `decoder` based on the voltage estimations and the power injection measurements in training data.
   \end{itemize}
   % 6th paragraph
   \item overview of evaluation results, highlight key findings:
   \begin{itemize}
       \item \textbf{Experiment setup}: test cases are IEEE 57, 118 systems; power demands are from GEFCom 2012 real-world load data.
       \item \textbf{The bus estimation accuracy}:\\
       a) Average Results see~\autoref{tab:inverse_meanae}.\\
       b) The distribution of percentage errors are~\autoref{fig:57_inverse_CDF} and ~\autoref{fig:118_inverse_CDF}.\\
       c) The upper bound of 95\% estimation errors are~\autoref{tab:inverse_95pe}.\\
       d) The estimation plot at a randoms time slot are~\autoref{fig:118_U_prediction} and ~\autoref{fig:118_W_prediction}.\\
       \textbf{Takeaways:} \\
       Our physics-guided neural networks have the best accuracy performance than other data-driven methods. \\
       Compared with MLP method, the superior performance of our physics-guided neural networks indicates that, by joint training, the "decoder" part captures domain knowledge (i.e. the Kirchhoff’s laws), informs the MLPNN 'encoder' part of physical laws, and helps improve its performance.
       \item \textbf{The bus estimation accuracy's robustness to data outliers} see ~\autoref{fig:118_inverse_outlier}\\
       \textbf{Takeaways:} Our physics-guided neural networks continuously perform best and are robust enough even for 10\% outliers in training data.
       \item \textbf{The computation time to solve power flow problems} see ~\autoref{tab:compute_time}\\
       \textbf{Takeaways:} The computation time of physics-guided NN is much faster than Newton (numerical) method, and physics-guided NN can be used to solve power flow problem nearly in real time.
       
       \item \textbf{TODO}:\\
       \textbf{How to evaluate our methods respecting the physical laws and other data-driven methods not?}\\
       i) \textbf{By inequality constraints}: evaluate how many voltages or reactive power injections falls in valid intervals? Typically there are inequality constraints on reactive power injection at PV buses and voltage magnitudes at PQ buses.\\
       ii) \textbf{By equality constraints}: power injection reconstruction errors? \\
       Power injection reconstruction errors in terms of mean absolute error (i.e. the prediction accuracy of `decoder`):\\
       On IEEE 57, MLP+MLP is 0.00479; MLP+BNN is 0.00697;\\
       On IEEE 118, MLP+MLP is 0.0437; MLP+BNN is 0.0716.\\
       The termination tolerance of Matpower is 1e-8. The reconstruction error maybe cannot be as small as 1e-8. Maybe skip this evaluation.\\
   \end{itemize}
   % 7th paragraph
   \item list our contributions:
   \begin{itemize}
    \item We propose physics-guided methods to solve power flow problems based on system measurement data. Our methods consider power flow physics and do not require additional knowledge of the power grid. 
    \item We evaluate our model using standard datasets and achieved better accuracy compare to previous methods. 
    \item Our physics-guided neural networks can serve as a power flow solver with fast computation time and good accuracy when power flow equations are inaccurate, out-of-date, or unknown and numerical methods can not apply. 
   \end{itemize}
\end{enumerate}

%%
\begin{table*}
    \caption{Bus Voltage Estimation Average Results}
    \centering
    \input{tables/inverse-mapping-average-results.tex}
    \label{tab:inverse_meanae}
\end{table*}
%%
%%
\begin{table*}
    \caption{The Upper Bound of 95\% Estimation Errors of Bus Voltage Estimation}
    \centering
    \input{tables/inverse-mapping-error-bound.tex}
    \label{tab:inverse_95pe}
\end{table*}
%%
%%
\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/57U_pe_cdf.pdf}
    \centering
    \vspace{-2mm}
    \caption{CDFs of absolute percentage errors of voltage real part (U)}
    \label{fig:57_U_CDF}
    \end{subfigure}
    %
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/57W_pe_cdf.pdf}
    \centering
    \vspace{-2mm}
    \caption{CDF of absolute percentage errors of voltage imaginary part (W)}
    \label{fig:57_W_CDF}
    \end{subfigure}
    \caption{CDF of absolute percentage errors of Bus Voltage Estimation on IEEE 57}
    \label{fig:57_inverse_CDF}
\end{figure}
%%
\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/118U_pe_cdf.pdf}
    \centering
    \vspace{-2mm}
    \caption{CDFs of absolute percentage errors of voltage real part (U)}
    \label{fig:118_U_CDF}
    \end{subfigure}
    %
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/118W_pe_cdf.pdf}
    \centering
    \vspace{-2mm}
    \caption{CDF of absolute percentage errors of voltage imaginary part (W)}
    \label{fig:118_W_CDF}
    \end{subfigure}
    \caption{CDF of absolute percentage errors of Bus Voltage Estimation on IEEE 118}
    \label{fig:118_inverse_CDF}
\end{figure}
%
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/118U_pred.pdf}
    \caption{Voltage real parts (U) estimation results of IEEE 118 case at a random timeslot}
    \label{fig:118_U_prediction}
\end{figure*}
%
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/118W_pred.pdf}
    \caption{Voltage imaginary parts (W) estimation results of IEEE 118 case at a random timeslot}
    \label{fig:118_W_prediction}
\end{figure*}
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/IEEE118_inverse_outlier.pdf}
    \caption{Bus Voltage Estimation Accuracy of Data-driven Methods with different level of outliers in training data}
    \label{fig:118_inverse_outlier}
\end{figure}
%
%%
\begin{table*}
    \caption{The Computation Time to Solve Power Flow Problems}
    \centering
    \input{tables/time.tex}
    \label{tab:compute_time}
\end{table*}
%%


==> tables/GB-estimation.tex <==
\begin{tabular}{c|c||c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{2}{|c}{RMSE}\\
 \hline
 Test Case& Admittance & BNN & TPBNN\\
 \hline
 \multirow{2}{*}{IEEE 57} & G & 2.36 & 0.263 \\
 & B & 4.71 & 0.260\\
 \hline
 \multirow{2}{*}{IEEE 118} & G & 1.61 & 0.197 \\
 & B & 8.19 & 0.971\\
 \hline
\end{tabular}

==> tables/forward-mapping-error-bound.tex <==
\begin{tabular}{c|c||c|c|c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{4}{|c}{95\% Absolute Percentage Errors (\%)} \\
 \hline
 Test Case& Power &LR & SVR & MLP & BNN\\
 \hline
 \multirow{2}{*}{IEEE 57} & P & 41.171 &27.600& 16.962 & 2.989\\
 & Q & 157.844 &64.798& 31.198 & 3.749\\
 \hline
 \multirow{2}{*}{IEEE 118} & P & 30.608 &18.916 & 8.733 & 3.689\\
 & Q & 122.775 &110.746& 45.815 & 5.737\\
 \hline
\end{tabular}

==> tables/forward-mapping-results.tex <==
\begin{tabular}{c|c||c|c|c|c||c|c|c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{4}{|c||}{Mean Absolute Error} & \multicolumn{4}{|c}{Maximum Absolute Error}\\
 \hline
 Test Case& Power &LR & SVR & MLPNN & BNN  &LR & SVR & MLPNN & BNN\\
 \hline
 %\multirow{2}{*}{IEEE 5} & P  & 0.0303 &AFG&   004 & 4& 5& 0.280& 2& 3 & 4 &5\\
 %& Q & 0.418 &AFG&   004 & 4& 5& 4.180 & 2& 3 & 4 &5\\
 %\hline
 \multirow{2}{*}{IEEE 57} & P & 0.142 &0.0786& 0.0544 & 0.00914&
 1.167 & 0.456& 0.599 & 0.125\\
 & Q & 0.314 &0.118& 0.0578 & 0.00732&
 3.740 & 1.294& 1.453 & 0.132\\
 \hline
 \multirow{2}{*}{IEEE 118} & P & 0.233 &0.158&  0.0898 & 0.0207&
 4.238 & 2.600& 1.471 & 0.400\\
 & Q & 0.598 &0.286& 0.0966 & 0.0383 &
 15.528& 9.360& 6.085 & 1.653\\
 \hline
 %\multirow{2}{*}{IEEE 123} & P &  0.0506 &AFG&   004 & 4& 5& 0.445 & 2& 3 & 4 &5\\
 %& Q & 0.0506 &AFG&   004 & 4& 5& 0.445& 2& 3 & 4 &5\\
%\hline
\end{tabular}

==> tables/inverse-interpolation.tex <==
\begin{tabular}{c|c|c||c|c|c|c|c|c}
\hline
\multicolumn{3}{c||}{ } & \multicolumn{6}{|c}{Root Mean Squared Error (p.u.)}\\
 \hline
  & Case& V &LR & SVR & MLP & MLP+MLP & MLP+BNN & MLP+TPBNN\\
 \hline
 %interpolation
 \multirow{4}{*}{Interpolation} & \multirow{2}{*}{IEEE 57} & $\boldsymbol{\mu}$ & $2.56\times10^{-2}$ & & $9.93\times10^{-3}\pm1.36\times10^{-3}$ & e-3 & e-3 & e-3\\
 & &$\boldsymbol{\omega}$ &$1.30\times10^{-2}$ & e-3& $1.26\times10^{-2}\pm4.87\times10^{-4}$ & e-3 & e-3 & e-3\\
 \cline{2-9}
 & \multirow{2}{*}{IEEE 118} & $\boldsymbol{\mu}$ & $8.96\times10^{-2}$ & e-2& $4.85\times10^{-2}\pm1.10\times10^{-3}$ & e-3 & e-3 & e-3\\
 & & $\boldsymbol{\omega}$ & $9.42\times10^{-2}$ & e-2& $3.75\times10^{-2}\pm3.61\times10^{-4}$ & e-3 & e-3 & e-3\\
 \hline
 % extrapolation
 \multirow{4}{*}{Extrapolation} & \multirow{2}{*}{IEEE 57} & $\boldsymbol{\mu}$ & $4.92\times10^{-2}$ & & $1.77\times10^{-2}\pm6.84\times10^{-4}$ & $8.70\times10^{-3}\pm5.57\times10^{-4}$ & $2.67\times10^{-3}\pm3.32\times10^{-4}$ & $2.48\times10^{-3}\pm3.04\times10^{-4}$\\
 & & $\boldsymbol{\omega}$ & $1.66\times10^{-2}$ & e-3& $1.90\times10^{-2}\pm1.48\times10^{-3}$ & $4.74\times10^{-3}\pm4.18\times10{-4}$ & $1.97\times10^{-3}\pm2.71\times10^{-4}$ & $1.89\times10^{-3}\pm3.00\times10^{-4}$\\
 \cline{2-9}
 & \multirow{2}{*}{IEEE 118} & $\boldsymbol{\mu}$ & $1.09\times10^{-1}$ & e-2& $3.47\times10^{-2}\pm1.56\times10^{-3}$ & $8.15\times10^{-3}\pm7.57\times10^{-5}$ & $6.88\times10^{-3}\pm8.58\times10^{-5}$ & $8.47\times10^{-3}\pm1.05\times10^{-4}$\\
 & & $\boldsymbol{\omega}$ & $9.12\times10^{-2}$ & e-2& $2.88\times10^{-2}\pm3.85\times10^{-4}$ & $1.15\times10^{-2}\pm1.10\times10^{-4}$ & $8.75\times10^{-3}\pm1.16\times10^{-4}$ & $1.30\times10^{-2}\pm7.61\times10^{-5}$\\
 \hline
\end{tabular}

==> tables/inverse-mapping-error-bound.tex <==
\begin{tabular}{c|c||c|c|c|c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{5}{|c}{95\% Absolute Percentage Errors (\%)} \\
 \hline
 Test Case& Voltage &LR & SVR & MLP & MLP+MLP& MLP+BNN\\
 \hline
 \multirow{2}{*}{IEEE 57} & U & 5.556 &0.781& 1.897 & 0.291 & 0.257\\
 & W & 62.065 &39.964& 48.723 & 6.102 & 8.407\\
 \hline
 \multirow{2}{*}{IEEE 118} & U & 18.316 &7.957 & 6.457 & 2.437 & 1.599\\
 & W & 57.156 &29.073& 25.081 & 8.930 & 5.200\\
 \hline
\end{tabular}

==> tables/inverse-mapping-results-10-noise.tex <==
\begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{5}{|c||}{Mean Absolute Error} & \multicolumn{5}{|c}{Maximum Absolute Error}\\
 \hline
 Test Case& Power &LR & SVR & MLPNN & MLP-MLP & BNN-MLP &LR & SVR & MLPNN & PY-MLP & TP-BNN\\
 \hline
 \multirow{2}{*}{IEEE 57} & U & 1 &0& 0 & 0.00230 & 5&
 0 & 0& 0 & 0.0994 &5\\
 & W & 0 &0& 0 &0.00679 & 5&
 0 & 0& 0 & 0.147 &5\\
 \hline
 \multirow{2}{*}{IEEE 118} & U & 0 &0& 0 &0.00993 & 5&
 1 & 0& 0 & 0.606 &5\\
 & W & 0 &0& 0 & 0.0120 & 5&
 0& 0 & 0 & 0.387 &5\\
 \hline
\end{tabular}

==> tables/inverse-mapping-results-15-noise.tex <==
\begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{5}{|c||}{Mean Absolute Error} & \multicolumn{5}{|c}{Maximum Absolute Error}\\
 \hline
 Test Case& Power &LR & SVR & MLPNN & MLP-MLP & BNN-MLP &LR & SVR & MLPNN & PY-MLP & TP-BNN\\
 \hline
 \multirow{2}{*}{IEEE 57} & U & 1 &0& 0 & 0.00319 & 5&
 0 & 0& 0 & 0.100  &5\\
 & W & 0 &0& 0 &0.00950 & 5&
 0 & 0& 0 & 0.138 &5\\
 \hline
 \multirow{2}{*}{IEEE 118} & U & 0 &0& 0.0188 &0.0141 & 5&
 1 & 0& 0.889 & 0.612 &5\\
 & W & 0 &0& 0.0192 & 0.0175 & 5&
 0& 0 & 0.554 & 0.390 &5\\
 \hline
\end{tabular}

==> tables/inverse-mapping-results-8-outlier.tex <==
\begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
\hline
% 20% noise
\multicolumn{2}{c||}{ } & \multicolumn{5}{|c||}{Mean Absolute Error} & \multicolumn{5}{|c}{Maximum Absolute Error}\\
 \hline
 Test Case& Power &LR & SVR & MLPNN & MLP-MLP & BNN-MLP &LR & SVR & MLPNN & PY-MLP & TP-BNN\\
 \hline
 \multirow{2}{*}{IEEE 57} & U & 1 &0& 0.00650 & 0.00353 & 5&
 0 & 0& 0.282 & 0.120 &5\\
 & W & 0 &0& 0.00988 &0.0109 & 5&
 0 & 0& 0.136 & 0.141 &5\\
 \hline
 \multirow{2}{*}{IEEE 118} & U & 0.0375 &0& 0.0349 &0.0140 & 5&
 1 & 0& 1.017 & 0.660 &5\\
 & W & 0.0307 &0& 0.0270 & 0.0192 & 5&
 0& 0 & 0.558 & 0.392 &5\\
 \hline
\end{tabular}

==> tables/inverse-mapping-results.tex <==
\begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{5}{|c||}{Mean Absolute Error} & \multicolumn{5}{|c}{Maximum Absolute Error}\\
 \hline
 Test Case& Power &LR & SVR & MLP & MLP+MLP & MLP+BNN &LR & SVR & MLP & MLP+MLP & MLP+BNN\\
 \hline
 %\multirow{2}{*}{IEEE 5} & U  & 0.00293 &AFG&   004 & 4& 5& 0.0494& 2& 3 & 4 &5\\
 %& W & 0.00202 &AFG&   004 & 4& 5& 0.0217 & 2& 3 & 4 &5\\
 %\hline
 \multirow{2}{*}{IEEE 57} & U & 0.0193 &0.00336& 0.00662 & 0.00113 & 0.000807&
 0.371 & 0.152& 0.273 & 0.0928 &0.0937\\
 & W & 0.00913 &0.00416& 0.00653 &0.000682 & 0.000903&
 0.219 & 0.111& 0.128 & 0.0959 &0.0965\\
 \hline
 \multirow{2}{*}{IEEE 118} & U & 0.0475 &0.0204& 0.0212 &0.00563 & 0.00404&
 1.858 & 0.972& 0.771 & 0.531 &0.501\\
 & W & 0.0361 &0.0291& 0.0195 & 0.00634 & 0.00413&
 0.992& 0.630 & 0.502 & 0.463 &0.450\\
 \hline
% \multirow{2}{*}{IEEE 123} & U &  0.0235 &AFG&   004 & 4& 5& 0.0764 & 2& 3 & 4 &5\\
% & W & 0.000933 &AFG&   004 & 4& 5& 0.00792 & 2& 3 & 4 &5\\
%\hline
\end{tabular}

==> tables/time.tex <==
\begin{tabular}{c|c||c|c|c|c|c|c}
\hline
\multicolumn{2}{c||}{ } & \multicolumn{6}{|c}{Time (s)}\\
 \hline
 Case& Test Data Size & Newton &LR & SVR & MLP & MLP+MLP & MLP+BNN\\
 \hline
IEEE 57 & 11419 & 85.64 & 9.84e-3 & 17.52 & 2.15e-2 & 7.15e-2 & 0.158\\
 \hline
IEEE 118 & 11419 & 171.28 & 2.66e-2 & 125.69 & 0.164 & 7.82e-2 & 0.272\\
 \hline
\end{tabular}
